Single Shot Structured Pruning Before Training

We introduce a method to speed up training by 2x and inference by 3x in deep neural networks using structured pruning applied before training. Unlike previous works on pruning before training which prune individual weights, our work develops a methodology to remove entire channels and hidden units with the explicit aim of speeding up training and inference. We introduce a compute-aware scoring mechanism which enables pruning in units of sensitivity per FLOP removed, allowing even greater speed ups. Our method is fast, easy to implement, and needs just one forward/backward pass on a single batch of data to complete pruning before training begins.

==> sections/table_cifar100.tex <==
\begin{table}[ht]
    \centering
    \caption{Accuracy of 3SP (in grey) compared to SNIP and GraSP for VGG19 on CIFAR100. Note that unstructured methods do not reduce compute cost. The original model obtains 72.4\% accuracy.}
      \begin{tabular}{llcccccc}
            \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Method}}  & \multicolumn{3}{c}{Parameters Pruned} \\ \cmidrule(l){3 -5} \cmidrule(l){6 -8}
            \multicolumn{2}{c}{}                                     & 80\%                & 90\%                   & 95\% \\
            \midrule
            Unstructured            & Uniform                         & 70.3 $\pm$ 0.16 \%  & 68.1 $\pm$ 0.11 \%     & 64.7 $\pm$ 0.27 \% \\
                                    & SNIP                           & 72.8 $\pm$ 0.10 \%  & 72.4 $\pm$ 0.08 \%     & 70.7 $\pm$ 0.11 \% \\
                                    & GraSP                          & 71.2 $\pm$ 0.08 \%  & 70.6 $\pm$ 0.15 \%     & 69.5 $\pm$ 0.07 \% \\
            \midrule
            Structured              & Uniform                        & 67.5 $\pm$ 0.16 \%  & 63.8 $\pm$ 0.13 \%     & 60.1 $\pm$ 0.29 \% \\
            \rowcolor{ourmethod}
                                    & 3SP                            & 69.9 $\pm$ 0.14 \%  & 68.3 $\pm$ 0.12 \%     & 63.2 $\pm$ 0.52 \% \\
            \rowcolor{ourmethod}
                                    & 3SP + re-init                  & 70.3 $\pm$ 0.16 \%  & 69.0 $\pm$ 0.08 \%     & 64.2 $\pm$ 0.35 \% \\
            \rowcolor{ourmethod}
                                    & 3SP + re-scale                 & 70.5 $\pm$ 0.13 \%  & 69.2 $\pm$ 0.11 \%     & 63.5 $\pm$ 0.63 \% \\
            \bottomrule
      \end{tabular}
      \label{table:CIFAR100}
    \end{table}

